In-Context Deep Learning via Transformer Models

We investigate the transformer's capability to simulate the training process of deep models via in-context learning (ICL), i.e., in-context deep learning. Our key contribution is providing a positive example of using a transformer to train a deep neural network by gradient descent in an implicit fashion via ICL. Specifically, we provide an explicit construction of a $(2N+4)L$-layer transformer capable of simulating $L$ gradient descent steps of an $N$-layer ReLU network through ICL. We also give the theoretical guarantees for the approximation within any given error and the convergence of the ICL gradient descent. Additionally, we extend our analysis to the more practical setting using Softmax-based transformers. We validate our findings on synthetic datasets for 3-layer, 4-layer, and 6-layer neural networks. The results show that ICL performance matches that of direct training.

==> 2method.tex <==







==> 3_2_ICL_short.tex <==


For using neural networks to approximate \eqref{eqn:loss}, which contains smooth functions changeable, we need to approximate these smooth functions by simple combination of activation functions.  
Our key approximation theory is using a sum of ReLUs to approximate any smooth function \cite{bai2023transformers}.

\begin{definition}[Approximability by Sum of ReLUs, Definition 12 of \cite{bai2023transformers}]
\label{def:sum_of_relus}
Let $z\in \R^k$.
We say that a function $g:\R^k \rightarrow \R$ is $(\epsilon_{\text{approx}}, R, H, C)$-approximable by sum of ReLUs if there exist a ``$(H,C)$-sum of ReLUs'' function $f_{H,C}(z)$ defined as
\begin{align*}
f_{H,C}(z) = \sum_{h=1}^{H} c_h \sigma(a_h^{\top} [z; 1]) 
\quad \text{with} \quad
\sum_{h=1}^{H} |c_h| \leq C, 
\quad \max_{h \in [H]} \|a_h\|_1 \leq 1, 
\quad a_h \in \R^{k+1}, \quad c_h \in \R,
\end{align*} 
such that $\sup_{z \in [-R, R]^k} |g(z) - f_{H,C}(z)| \leq \epsilon_{\rm approx}$.
\end{definition}



\textbf{Overview of Our Proof Strategy.}
\cref{lem:decomposition_gd} and \cref{def:sum_of_relus} motivate the following strategy: term-by-term approximation for our gradient descent step \eqref{eqn:decomposition_gd}. 

\begin{enumerate}[leftmargin=3.5em]
    \item [\textbf{Step 1.}]
    Given $(x_i,w)$, we use $N$ attention layers to approximate the output of
    the first $j$ layers with input $x_i$, $p_i(j)\coloneqq {\rm pred}_h(x_i ; j) \in \R^k$ (\cref{def:N_nn}) for any $j \in [N]$. 
    Then we use $1$ attention layer to approximate \red{chain-rule intermediate terms} $r'_i(j)[k] := 
    r'(v_{k_{j+1}}^\top p_i(j))$ (\cref{def:abbv}) for any 
    $i \in [n]$, $j \in [N-1] $ and $k \in [K]$: \cref{lem:aprox_p} and \cref{lem:aprox_r_p}.
    \item [\textbf{Step 2.}]
    Given $(r'_i, p_i, w)$, we use an MLP layer to approximate 
    $\partial_1 \ell(p_i(N),y_i)$ (\cref{lem:decomposition_gd}), for $i \in [n]$, and use $N$ element-wise multiplication layers to approximate $s_i(j)$ (\cref{def:abbv}) and $\partial_1 \ell(p_i(N),y_i) \cdot s_i(j)$, for any 
    $j \in[N]$: 
    \cref{lem:aprox_pl},
    \cref{lem:aprox_s_j} and \cref{lem:aprox_g_s_j}.
    Moreover, \cref{lem:error_gs} shows the closeness result for
    approximating $\partial_1 \ell(p_i(N),y_i) \cdot s_i(j)$, which leads to the final error accumulation in \cref{thm:icl_gd}.
    \item [\textbf{Step 3.}]
    Given $(p_i, r'_i, g_i s_i(j), w)$, we use an attention layer to approximate $w - \eta \nabla \mathcal{L}_n(w)$.
    Then we use an MLP layer to approximate ${\rm Proj}_{\mathcal{W}}(w)$.
    And implementing $L$ steps gradient descent by a 
    $(2N+4)L$-layer neural network
    ${\rm NN}_{\theta}$ 
    constructed based on 
    \textbf{Step 1 and 2}.
    Finally, we arrive our main result: \cref{thm:icl_gd}. 
    Furthermore, \cref{lem:error_general} shows closeness results to the true gradient descent path. 
\end{enumerate}

\textbf{Step 1.}
We start with approximation for $p_i(j)$.
\begin{lemma}[Approximate $p_i(j)$]
    \label{lem:aprox_p}
    Let upper bounds $B_v, B_x, B_u > 0$ such that
    for any $k \in [K], j \in [N] ~\text{and}~ i \in [n]$, $\|v_{k_j}\|_2 \leq B_v$,
    $\|u\|_2 \leq B_u$ and $\|x_i\|_2 \leq B_x$.
    For any $j \in [N], i \in [n]$, define
    \begin{align}
    \label{eqn:b_r}
        B_r^j :=  \max_{\abs{t} \leq B_v B_r^{j-1}} \abs{r(t)},
        \quad B_r^0 := B_x ,\quad\text{and}\quad
        B_r := & ~ \max_{j} B_r^j.
    \end{align}
    Let function $r(t)$ be $(\epsilon_r, R_1, M_1, C_1)$-approximable for $R_1 = \max \{B_v B_r, 1\}$, $M_1 \leq \Tilde{\mathcal{O}}(C_1^2 \epsilon_r^{-2})$, where $C_1$ depends only on $R_1$ and the $C^2$-smoothness of $r$.
    Then, for any $\epsilon_r>0$, there exist $N$ attention layers ${\rm Attn}_{\theta_1}, \ldots, {\rm Attn}_{\theta_N}$ such that for any input $h_i \in \R^D$ takes from \eqref{eqn:input}, they map
    \begin{align*}
        h_i = [x_i; y_i; w; \bar{p}_i(1); \ldots; \bar{p}_i(j-1); \mathbf{0}; 1; t_i] \xrightarrow
        {{\rm Attn}_{\theta_j}} 
        \Tilde{h_i} = [x_i; y_i; w; \bar{p}_i(1); \ldots; \bar{p}_i(j); \mathbf{0}; 1; t_i],
    \end{align*}
    where $\bar{p}_i(j)$ is  approximation for $p_i(j)$ (\cref{def:N_nn}).
    In the expressions of $h_i$ and $\Tilde{h}_i$, the dimension of $\mathbf{0}$ differs.
    Specifically, the $\mathbf{0}$ in $h_i$ is larger than in $\Tilde{h}_i$.
    The dimensional difference between these $\mathbf{0}$ vectors equals the dimension of $\bar{p}_i(j)$.
    Suppose function $r$ is $L_r$-smooth in bounded domain $\mathcal{W}$, then for any $i \in [n+1]$, $j \in [N]$, $\bar{p}_i(j)$ such that
    \begin{align}
    \label{eqn:error_1}
        \bar{p}_i(j) = p_i(j) + \epsilon(i,j), \quad  \|\epsilon(i,j)\|_2 \leq 
        \begin{cases}
            (\sum_{l=0}^{j-1} 
            K^{l/2} L_r^l B_v^l) \sqrt{K} \epsilon_r ~,   \quad 1 \leq j \leq N-1 \\ 
            (\sqrt{K} B_u \sum_{l=0}^{N-2} 
            K^{l/2} L_r^l B_v^l) \epsilon_r 
            ~,  \quad j=N
        \end{cases}.
    \end{align} 
    Additionally, for any $j \in [N]$, the norm of parameters $\|\theta_{j}\|$ defined as \eqref{eqn:tf_norm}  such that
    \begin{align*}
        \|\theta_{j}\| \leq 
        \begin{cases}
            1 + K C_1, & j \neq N \\
            1 + 2K, & j = N.
        \end{cases}
    \end{align*}
\end{lemma}
\begin{proof}[Proof Sketch]
    By \cref{def:N_nn}, we provide term-by-term approximations for $p_i(j)$ as forward propagation. 
    Specifically, we construct Attention layers to implement forward propagation algorithm.
    Then we establish upper bounds for the errors $\|\bar{p}_i(j) - p_i(j)\|_2$ inductively. Finally, we present the norms \eqref{eqn:tf_norm} of the Transformers constructed.
    Please see \cref{proof:lem:aprox_p} for a detailed proof.
\end{proof}

Notice that the form of error accumulation in \cref{lem:aprox_p} is complicated. 
For the ease of later presentations, we define the upper bound of coefficient in \eqref{eqn:error_1} as 
\begin{align}
\label{eqn:E_r}
    E_r := \max_{1 \leq j \leq N}
    \frac{\|\epsilon(i,j)\|_2}{\epsilon_r}
    = \max_{1 \leq j \leq N}
    \{(\sum_{l=0}^{j-1} 
    K^{l/2} L_r^l B_v^l) \sqrt{K}, \sqrt{K} B_u \sum_{l=0}^{N-2} 
    K^{l/2} L_r^l B_v^l\},
\end{align}
such that  \eqref{eqn:error_1} becomes
\begin{align}        \label{eqn:e_r}
        \bar{p}_i(j) = p_i(j) + \epsilon(i,j), \quad  \|\epsilon(i,j)\|_2 \leq 
        E_r \epsilon_r.
\end{align}
Moreover, we abbreviate $\bar{p}_i := [\bar{p}_i(1); \ldots; \bar{p}_i(N)] \in \R^{NK}$,
such that the output of ${\rm Attn}_{\theta_1} \circ \cdots \circ {\rm Attn}_{\theta_N}$ is 
    \begin{align}
        h_i = [x_i; y_i; w; \bar{p}_i; \mathbf{0}; 1; t_i].
        \label{eqn:h_i_p}
    \end{align}
Then, the next lemma approximates $r'_i(j)$ base on $\bar{p}_i(j)$ obtained in \cref{lem:aprox_p}.

\begin{lemma}[Approximate $r'_i(j)$]
    \label{lem:aprox_r_p}
    Let upper bounds $B_v, B_x, B_u > 0$ such that
    for any $k \in [K], j \in [N] ~\text{and}~ i \in [n]$, $\|v_{k_j}\|_2 \leq B_v$,
    $\|u\|_2 \leq B_u$ and $\|x_i\|_2 \leq B_x$.
    For any $j \in [N], i \in [n]$, define
    \begin{align*}
        B_r'^j :=  \max_{\abs{t} \leq B_v B_{r'}^{j-1}} \abs{r'(t)},
        \quad B_{r'}^0 := B_x,\quad\text{and}\quad
        B_{r'} :=  \max_{j} B_{r'}^j.
    \end{align*}
    Suppose function $r'(t)$ is $(\epsilon_{r'}, R_2, M_2, C_2)$-approximable for $R_2 = \max \{B_v B_{r'}, 1\}$, $M_2 \leq \Tilde{\mathcal{O}}(C_2^2 \epsilon_r'^{-2})$, where $C_2$ depends only on $R_2$ and the $C^2$-smoothness of $r'$.
    Then, for any $\epsilon_r > 0$, there exist an attention layer 
    $ {\rm Attn}_{\theta_{N+1}}$ such that for any input $h_i \in \R^D$ takes from \eqref{eqn:h_i_p}, it maps
    \begin{align*}
        h_i = [x_i; y_i; w; \bar{p}_i; \mathbf{0}; 1; t_i] \xrightarrow
        {{\rm Attn}_{\theta_{N+1}}} 
        \Tilde{h_i} = [x_i; y_i; w; \bar{p}_i; \bar{r}'_i; \mathbf{0}; 1; t_i],
    \end{align*}
    where $\bar{r}'_i(j)$ is  approximation for $r'_i(j)$ (\cref{def:abbv}) and $\bar{r}'_i := [\bar{r}'_i(1); \ldots; \bar{r}'_i(N-1)] \in \R^{(N-1)K}$.
    Similar to \cref{lem:aprox_p}, in the expressions of $h_i$ and $\Tilde{h}_i$, the dimension of $\mathbf{0}$ differs.
    In addition, let $E_r$ be defined in \eqref{eqn:e_r}, for any $i \in [n+1]$, $j \in [N], k \in [K]$, $\bar{r}'_i(j)$ such that 
    \begin{align}
        \bar{r}'_i(j)[k] = r'_i(j)[k] + \epsilon(i,j,k), \quad  \abs{\epsilon(i,j,k)} \leq 
        \epsilon_{r'} +
        L_{r'} B_v E_r \epsilon_r,
        \label{eqn:error_2}
    \end{align}
    where $\epsilon_r$ denotes the error generated in approximating
    $r$ by sum of ReLUs $\bar{r}$ follows \eqref{eqn:r_bar}.
    Additionally, the norm of parameters $\|\theta_{N+1}\|$ defined as \eqref{eqn:tf_norm} such that
    $\|\theta_{N+1}\| \leq
    1 + K (N-1) C_2$.
\end{lemma}
\begin{proof}[Proof Sketch]
    By \cref{lem:aprox_p}, we obtain $\bar{p}_i(j)$, the approximation for $p_i(j)$ \eqref{eqn:p}.
    Using $\bar{p}_i(j)$, we construct an Attention layer to approximate $r'_i(j)$.
    We then establish upper bounds for the errors $\abs{\bar{r}'_i(j)[k] - 
    r'_i(j)[k]}$ by applying Cauchy-Schwarz inequality and \cref{lem:aprox_p}.
    Finally we present the norms \eqref{eqn:tf_norm} of the Transformers constructed.
    Please see \cref{proof:lem:aprox_r_p} for a detailed proof.
\end{proof}


Let ${\rm Attn}_{\theta_j}
(j \in [N])$ be as defined in \cref{lem:aprox_p}, then \cref{lem:aprox_r_p} implies that for the input takes from \cref{prob:icl_n}, the output of ${\rm Attn}_{\theta_1} \circ \cdots \circ {\rm Attn}_{\theta_{N+1}}$ is 
\begin{align}
    h_i = [x_i; y_i; w; \bar{p}_i; \bar{r}'_i; \mathbf{0}; 1; t_i].
    \label{eqn:h_i_r}
\end{align}

\textbf{Step 2.} Now, we use the above lemmas to construct an approximation for $\partial_1 \ell(p_i(N),y_i)$.

\begin{lemma}[Approximate 
$\partial_1 \ell(p_i(N),y_i)$]
    \label{lem:aprox_pl}
    Let upper bounds $B_v, B_x, B_u > 0$ such that
    for any $k \in [K], j \in [N] ~\text{and}~ i \in [n]$, $\|v_{k_j}\|_2 \leq B_v$,
    $\|u\|_2 \leq B_u$ and $\|x_i\|_2 \leq B_x$.
    Suppose function $\partial_1 \ell(t,y)$ be $(\epsilon_{l}, R_3, M_3, C_3)$-approximable for $R_3 = \max
    \{B_v B_r, 1\}$, $M_3 \leq \Tilde{\mathcal{O}}(C_3^2 \epsilon_l^{-2})$, where $C_3$ depends only on $R_3$ and the $C^3$-smoothness of $\partial_1 \ell$.
    Then, there exists an MLP layer 
    $ \rm{MLP}_{\theta_{N+2}}$ such that for any input sequences $h_i \in \R^D$ takes from \eqref{eqn:h_i_r}, 
    it maps
    \begin{align*}
        h_i = [x_i; y_i; w; \bar{p}_i; \bar{r}'_i; \mathbf{0}; 1; t_i] \xrightarrow
        {{\rm{MLP}}_{\theta_{N+2}}} 
        \Tilde{h_i} = [x_i; y_i; w; \bar{p}_i; \bar{r}'_i; g_i; \mathbf{0}; 1; t_i],
    \end{align*}
    where $g_i$ is an approximation for $\partial_1 \ell(p_i(N),y_i)$ such that
    \begin{align*}
        g_i = \partial_1 \ell(\bar{p}_i(N),y_i) + \epsilon(i), \quad\text{with}\quad
        \abs{\epsilon(i)} \leq \epsilon_l +
        L_l E_r \epsilon_r.
    \end{align*}
     Additionally, the parameters $\theta_{N+2}$ such that $\|\theta_{N+2}\| \leq
        \max \{R_3 +1, C_3\}$.
\end{lemma}
\begin{proof}[Proof Sketch]
    By \cref{lem:aprox_p}, we obtain $\bar{p}_i(N)$, the approximation for $p_i(N)$ \eqref{eqn:p}.
    Using $\bar{p}_i(N)$, we construct an MLP layer to approximate $\partial_1 \ell(p_i(N),y_i)$.
    We then establish upper bounds for the errors $\abs{g_i - \partial_1 \ell(p_i(N),y_i)}$ and present the norms \eqref{eqn:tf_norm} of Transformers constructed.
    Please see \cref{proof:lem:aprox_pl} for a detailed proof.
\end{proof}


Let ${\rm Attn}_{\theta_j}
(j \in [N+1])$ be as defined in \cref{lem:aprox_p} and \cref{lem:aprox_r_p}, then for any input sequences $h_i \in \R^D$ takes from \eqref{eqn:input}, the output of ${\rm Attn}_{\theta_1} \circ \cdots \circ {\rm Attn}_{\theta_{N+1}} \circ \rm{MLP}_{\theta_{N+2}}$ is 
\begin{align}
    h_i = [x_i; y_i; w; \bar{p}_i; \bar{r}'_i; \mathbf{0}; 1; t_i].
    \label{eqn:h_i_g}
\end{align}

Before introducing our next approximation lemma, we define an element-wise multiplication layer, since attention mechanisms and MLPs are unable to compute self-products (e.g., output $xy$ from input $[x; y]$).
To enable self multiplication, we introduce a function $\gamma$. 
This function, for any square matrix, preserves the diagonal elements and sets all others to zero.

\begin{definition}[Operator Function $\gamma$]
    \label{def:gamma}
    For any square matrix $A \in 
    \R^{n \times n}$, define $\gamma(A) := {\rm diag}(A[1,1], \ldots A[n,n]) \in \R^{n \times n}$.
\end{definition}

By \cref{def:gamma}, we introduce the following element-wise multiplication layer, capable of performing self-multiplication operations such as the Hadamard product.

\begin{definition}[Element-wise Multiplication Layer]
\label{def:ewml}
    Let $\gamma$ be defined as \cref{def:gamma}.
    An element-wise multiplication layer with $m$ heads is denoted as ${\rm Attn}_{\theta}(\cdot)$ with parameters $\theta=\{Q_m, K_m, V_m\}_{m \in [M]}$. 
    On any input sequence $H \in \R^{D \times n}$, 
\begin{align}
\label{eqn:ewml}
{\rm EWML}_{\theta}(H) = H +  \sum_{i=1}^m  (V_m H) \cdot \gamma((Q_m H)^{\top} 
(K_m H)).
\end{align}
where $Q_m,K_m,V_m\in\R^{D\times D}$ and $\gamma(\cdot)$ is operator function follows \cref{def:gamma}.
In vector form, for for each token $h_i\in\R^D$ in $H$, it outputs
$[{\rm EWML}_{\theta}(H)]_i = h_i +  \sum_{m=1}^M  \gamma (\langle Q_m h_i, K_m h_i \rangle) \cdot V_m h_i$.
In addition, we define $L$-layer neural networks 
${\rm EWML}_{\theta}^{L} := {\rm EWML}_{\theta_1} \circ \cdots \circ
{\rm EWML}_{\theta_L}$.
\end{definition}

\begin{remark}[Necessary for Element-Wise Multiplication Layer]
As we shall show in subsequent
sections, element-wise multiplication layer is capable of implementing multiplication in $h_i$. 
Specifically, it allows us to multiple some elements in $h_i$ in \cref{lem:aprox_s_j} and \cref{lem:aprox_g_s_j}.
By \cref{def:attn}, it is impossible for transformer layers to achieve our goal without any other assumptions.
\end{remark}
Similar to \eqref{eqn:tf_norm}, we define the norm for $L$-layer transformer 
${\rm EWML}_{\theta}^{L}$ as:
\begin{align}
\label{eqn:ewml_norm}
\| \theta \| :=  
\max_{m \in [M], l \in [L]} 
\left\{ \|Q_{m}^l\|_{\rm op}, 
\| K_{m}^l\|_{\rm op}, 
\| V_{m}^l\|_{\rm op} \right\}.
\end{align}
Then, given the approximations for $p_i(j)$ and $r'_i(j)$, we use $N-1$ element-wise multiplication layer (\cref{def:ewml}) to approximate $s_i(j)$, the chain-rule intermediate terms defined as \cref{def:s}.

\begin{lemma}[Approximate $\bar{s}_t(j)$]
    \label{lem:aprox_s_j}
    Recall that $s_i(j) = r'_i(j-1) \odot (V_{j+1}^{\top} \cdot s_i(j+1))$ follows \cref{def:s}. 
    Let the initial input takes from \eqref{eqn:h_i_g}.
    Then, there exist $N-1$ element-wise multiplication layers: ${\rm EWML}_{\theta_{N+3}}, \ldots, {\rm EWML}_{\theta_{2N+1}}$ such that for input sequences, 
    $j \in [N-1]$,
    \begin{align*}
        h_i = [x_i; y_i; w; \bar{p}_i; \bar{r}'_i; g_i; \bar{s}_i(N-1); \ldots; \bar{s}_i(j+1); \mathbf{0}; 1; t_i],
    \end{align*}
    they map ${\rm EWML}_{\theta_{2N+2-j}}(h_i)
        = [x_i; y_i; w; \bar{p}_i; \bar{r}'_i; g_i; \bar{s}_i(N-1); \ldots; \bar{s}_i(j); \mathbf{0}; 1; t_i]$,
    where the approximation $\bar{s}_i(j)$ is defined as recursive form: for any $i \in [n+1], j \in[N-1]$,
    \begin{align}
        \bar{s}_i(j) 
        := \bar{r}'_i(j-1) \odot (V_{j+1}^{\top} \cdot \bar{s}_i(j+1)).
        \label{eqn:s_bar_i(j)}
    \end{align}
    Additionally, for any $j \in [N-1]$,  $\|\theta_{N+2+j}\|$ defined in \eqref{eqn:tf_norm} satisfies $\|\theta_{N+2+j}\| \leq 1$.
\end{lemma}
\begin{proof}[Proof Sketch]
    By \cref{lem:aprox_p} and \cref{lem:aprox_r_p}, we obtain $\bar{p}_i(j)$ and $\bar{r}'_i(j)$, the approximation for $p_i(j)$ \eqref{eqn:p} and $r'_i(j)$ respectively.
    Using $\bar{p}_i(j)$ and $\bar{r}'_i(j)$, we construct $N-1$ element-wise multiplication layers to approximate $s_i(j)$.
    We then present the norms \eqref{eqn:ewml_norm} of the EWMLs constructed.
    Please see \cref{lem:aprox_s_j} for a detailed proof.
\end{proof}



Let ${\rm Attn}_{\theta_j}
(j \in [N+1]), {\rm MLP}_{\theta_{N+2}} $ be as defined in \cref{lem:aprox_p}, \cref{lem:aprox_r_p} and 
\cref{lem:aprox_g_s_j} respectively.
Define $\bar{s}_i := 
[\bar{s}_i(N-1); \ldots; \bar{s}_i(1)] \in \R^{(N-1)K}$, then for any input sequences $h_i \in \R^D$ takes from \cref{prob:icl_n}, the output of neural network
\begin{align}
    {\rm Attn}_{\theta_1} \circ \cdots \circ
    {\rm Attn}_{\theta_{N+1}}
    \circ
    {\rm MLP}_{\theta_{N+2}}
    \circ
    {\rm EWML}_{\theta_{N+3}}
    \circ \cdots \circ {\rm EWML}_{\theta_{2N+1}},  
    \label{eqn:nn_1}
\end{align}
is 
\begin{align}
    h_i = [x_i; y_i; w; \bar{p}_i; \bar{r}'_i; 
    \bar{s}_i; \mathbf{0}; 1; t_i].
    \label{eqn:h_i_s}
\end{align}
For the sake of simplicity, we consider  ReLU Attention layer and MLP layer are both a special kind of transformer.
Specifically, \red{the explanation}.
In this way, by \cref{def:tf}, \eqref{eqn:nn_1} becomes
\begin{align*}
 {\rm TF}_{\theta}^{N+2} \circ {\rm EWML}_{\theta}^{N-1}.    
\end{align*}
By \cref{lem:decomposition_gd} and \cref{def:s}, notice that finally we need to approximate 
\begin{align*}
    \sum_{i=1}^{n} g_i s_i(j) p_i(j-1),
\end{align*}
for any $i \in [n]$ and $j \in [N]$.
Moreover, it is difficult to construct attention layers that approximate the above terms explicitly.
Thus, before we go on to step three, we need to approximate $g_i s_i(j)$.

\begin{lemma}[Approximate $g_i \bar{s}_i(j)$]
    \label{lem:aprox_g_s_j}
    For any $i \in [n+1]$, suppose the input sequences $h_i = [x_i; y_i; w; \bar{p}_i; \bar{r}'_i; g_i; \bar{s}_i; \mathbf{0}; 1; t_i]$ takes from \eqref{eqn:h_i_s},
    then there exist an element-wise multiplication layer ${\rm EWML}_{\theta_{2N+2}}$ such that 
    ${\rm EWML}_{\theta_{2N+2}}(h_i)
        = [x_i; y_i; w; \bar{p}_i; \bar{r}'; g_i; g_i \bar{s}_i; \mathbf{0}; 1; t_i]$.
    Additionally, for any $j \in [N]$, the parameters $\theta_{j}$ such that $\|\theta_{2N+2}\| \leq 2$.
\end{lemma}

\begin{proof}[Proof Sketch]
    By \cref{lem:aprox_pl} and \cref{lem:aprox_s_j}, we obtain $g_i$ and $\bar{s}_i(j)$, the approximations for $\partial_1 \ell(p_i(N),y_i)$ (\cref{lem:decomposition_gd}) and $s_i(j)$ (\cref{def:s}), respectively.
    Using these we construct an element-wise multiplication layer to approximate $g_i \bar{s}_i(j)$.
    We then present the norms \eqref{eqn:ewml_norm} of the EWML  constructed. 
    Please see \cref{proof:lem:aprox_g_s_j} for a detailed proof.
\end{proof}



Next we calculate error $\abs{g_i \bar{s}_i(j)[k] - \partial_1 \ell(p_i(N),y_i) s_i(j)[k]}$ based on \cref{lem:aprox_r_p} and \cref{lem:aprox_pl}.

\begin{lemma}[Error for $g_i \bar{s}_i(j)$]
\label{lem:error_gs}
    Suppose the upper bounds $B_v, B_x, B_u > 0$ such that
    for any $k \in [K], j \in [N] ~\text{and}~ i \in [n]$, $\|v_{k_j}\|_2 \leq B_v$,
    $\|u\|_2 \leq B_u$ and $\|x_i\|_2 \leq B_x$.
    Let $r'_i(j) \in \R^K$ such that $r'_i(j)[k] := 
    r'(v_{k_{j+1}}^\top p_i(j))$ follows \cref{def:abbv}.
    Let $s_i(j) = R_i(j-1) V_{j+1}^{\top} \ldots R_i(N-3) V_{N-1}^{\top} \cdot R_i(N-2) u$ follows \cref{def:s}.
    Let $\bar{r}'_i(j), g_i, \bar{s}_i(j)$ be the approximations for $r'_i(j), \partial_1 \ell(p_i(N),y_i), s_i(j)$  follows
    \cref{lem:aprox_r_p},
    \cref{lem:aprox_pl} and \cref{lem:aprox_s_j} respectively.
    Let $B_{r'}$ be the upper bound of $\bar{r}'_i(j)[k]$ and $r'_i(j)[k]$ as defined in \cref{lem:aprox_r_p}.
    Let $B_l$ be the upper bound of $g_i$ and $\partial_1 \ell(p_i(N),y_i)$ as defined in \cref{lem:aprox_pl}.
    Then for any $i \in [n+1], j \in [N-1], k \in [K]$, 
    \begin{align*}
        & ~ \bar{s}_i(j)[k] 
        \leq  B_{r'}^{N-j} B_v^{N-j-1} B_u, \\
        & ~  \abs{\bar{s}_i(j)[k] -  s_i(j)[k]}  
        \leq (\epsilon_{r'} +
        L_{r'} B_v E_r \epsilon_r) B_v B_s [\sum_{l=1}^{N-n-2} (B_{r'} B_v \sqrt{K})^l] 
        + (B_{r'} B_v \sqrt{K})^{N-n-1} (\epsilon_{r'} +
        L_{r'} B_v E_r \epsilon_r) B_u. \\
        & ~  \abs{g_i \bar{s}_i(j)[k] - \partial_1 \ell(p_i(N),y_i) s_i(j)[k]} 
        \leq B_s \epsilon_l + B_l E_s \epsilon_{r'} + 
        (L_l B_s + B_l E_s L_{r'} B_v) E_r
        \epsilon_r,
    \end{align*}
    where 
    \begin{align}
        B_s := & ~ 
        \max_j \{B_{r'}^{N-j} B_v^{N-j-1} B_u\}, 
        \label{eqn:B_s} \\
        E_s := & ~ \max_j 
        \{ B_v B_s [\sum_{l=1}^{N-n-2} (B_{r'} B_v \sqrt{K})^l] + (B_{r'} B_v \sqrt{K})^
        {N-n-1} B_u \},
        \label{eqn:E_s}
    \end{align} 
    are the upper bound of $\bar{s}_i(j)[k]$ and
    coefficient of $\epsilon_{r}'$ in $\abs{\bar{s}_i(j)[k] - s_i(j)[k]}$, respectively.
\end{lemma}
\begin{proof}[Proof Sketch]
    By \cref{lem:aprox_g_s_j}, we manage to approximate
    $\partial_1 \ell (p_i(N),y_i) s_i(j)$ by $g_i \bar{s}_i(j)$.
    Applying the triangle inequality, we derive:
    $\abs{g_i \bar{s}_i(j)[k] - \partial_1 \ell(p_i(N),y_i) s_i(j)[k]} \leq \abs{g_i - \partial_1 \ell(p_i(N),y_i)} \cdot 
    \abs{\bar{s}_i(j)[k]} + \abs{g_i}\cdot \abs{\bar{s}_i(j)[k] - s_i(j)[k]}$.
    We bound the four terms separately.
    From \cref{lem:aprox_pl}  we know $\abs{g_i - \partial_1 \ell(p_i(N),y_i)}$ is bounded by $\epsilon_l +
    L_l E_r \epsilon_r$.
    We then use induction to establish upper bounds for $\bar{s}_i(j)[k]$ and $\abs{\bar{s}_i(j)[k] - s_i(j)[k]}$.
    Please see \cref{proof:lem:error_gs} for a detailed proof.
\end{proof}



\cref{lem:error_gs} offers the explicit form of the error $\abs{g_i \bar{s}_i(j)[k] - \partial_1 \ell(p_i(N),y_i) s_i(j)[k]}$, which is crucial for calculating the error $\|\nabla_w \bar{L}_n(w) - \nabla_w \mathcal{L}_n(w)\|_2$ in \cref{thm:icl_gd}.

\textbf{Step 3.} Combining the above, we prove the existence of a neural network, that implements $L$ in-context GD steps on our $N$-layer neural network. 
And finally we arrive our main result: a neural network $\mathcal{T}$ for \cref{prob:icl_n}.

\begin{theorem}[In-context gradient descent on $N$-layer NNs]
\label{thm:icl_gd}
    Fix any $B_v, B_u, \eta, \epsilon > 0, L \geq 1$.
    For any input sequences takes from $\eqref{eqn:input}$, their exist upper bounds $B_x,B_y$ such that for any $i \in [n]$, $\|y_i\|_2 \leq B_y$, $\|x_i\|_2 \leq B_x$.
    Suppose $\mathcal{W}$ is a closed domain such that
    for any $j \in [N-1], k \in [K]$,
    \begin{align*}
        \mathcal{W} \subset \{
        w = [v_{k_j};u_k] \in \R^{D_N}: \|v_{k_j}\|_2 \leq B_v, \|u_k\|_2 \leq B_u \},
    \end{align*}
    and ${\rm Proj}_{\mathcal{W}}$ project $w$ into bounded domain $\mathcal{W}$. 
    Assume
    ${\rm Proj}_{\mathcal{W}} = {\rm MLP}_{\theta}$ for some MLP layer with hidden dimension 
    $D_w$ parameters $\|\theta\| \leq C_{w}$.
    Then, for any $\epsilon > 0$, there exists a transformer model ${\rm NN}_{\theta}$ with $(2N+4)L$ hidden layers
    consists of $L$ neural network blocks 
    ${\rm TF}_{\theta}^{N+2} \circ
    {\rm EWML}_{\theta}^{N} \circ
    {\rm TF}_{\theta}^{2}$,
    \begin{align*}
        {\rm NN}_{\theta} := 
        {\rm TF}_{\theta}^{N+2} \circ
        {\rm EWML}_{\theta}^{N} \circ
        {\rm TF}_{\theta}^{2}
        \circ \ldots \circ 
        {\rm TF}_{\theta}^{N+2} \circ
        {\rm EWML}_{\theta}^{N} \circ
        {\rm TF}_{\theta}^{2},
    \end{align*}
    such that the heads number $M^l$, parameter dimensions $D^l$, and the parameter norms
    $\|\theta\|_2$ suffice
    \begin{align*}
        \max_{ l \in (2N+4)L} M^l \leq \Tilde{O}(\epsilon^{-2}), \quad
        \max_{ l \in (2N+4)L} D^l \leq \Tilde{O}(\epsilon^{-2}) + D_w, \quad
        \max_{ l \in (2N+4)L} \|\theta^l\| \leq 
        O(\eta) + C_w + 1,
    \end{align*}
    where $O(\cdot)$ hides the constants that depend on $K,N$, the radius parameters $B_x,B_y,B_u,B_v$ and the smoothness
    of $r$ and $\ell$. 
    And this neural network such that for any input sequences $H^{(0)}$, take from \eqref{eqn:input}, ${\rm NN_{\theta}}(H^{(0)})$ implements $L$ steps in-context gradient descent on risk Eqn~\eqref{eqn:loss}: For every $l \in [L]$, the $(2N+4)l$-th layer outputs $h_i^{((2N+4)l)} = [x_i; y_i; \bar{w}^{(l)}; \mathbf{0}; 1; t_i]$ for every $i \in [n+1]$, and approximation gradients
    $\bar{w}^{(l)}$ such that 
    \begin{align*}
        \bar{w}^{(l)} = 
        {\rm Proj}_{\mathcal{W}} 
        (\bar{w}^{(l-1)} - \eta \nabla \mathcal{L}_n(\bar{w}^{(l-1)}) + \epsilon^{(l-1)}), \; \bar{w}^{(0)} = \mathbf{0},
        \; \text{where $\|\epsilon^{(l-1)}\|_2 \leq \eta \epsilon$ is error term.}
    \end{align*}
\end{theorem}
\begin{proof}[Proof Sketch]
    Let the first $2N+2$ layers of ${\rm NN}_{\theta}$ are Transformers and EWMLs constructed in \cref{lem:aprox_p}, 
    \cref{lem:aprox_r_p},
    \cref{lem:aprox_pl},
    \cref{lem:aprox_s_j} and \cref{lem:aprox_g_s_j}.
    Explicitly, we design the last two layers to implement the gradient descent step (\cref{lem:decomposition_gd}).
    We then establish the upper bounds for error $\|\nabla_w \bar{L}_n(w) - \nabla_w \mathcal{L}_n(w)\|_2$, where $\nabla_w \bar{L}_n(w)$, derived from the outputs of ${\rm NN}_{\theta}$, approximates
    $\nabla_w \mathcal{L}_n(w)$.
    Next, for any $\epsilon>0$, we select appropriate parameters $\epsilon_l$, $\epsilon_r$ and $\epsilon_{r'}$ to ensure that  $\|\nabla_w \bar{L}_n(\bar{w}^{(l-1)}) - \nabla_w \mathcal{L}_n(\bar{w}^{(l-1)})\|_2 
    \leq \epsilon$ holds for any $l \in [L]$.
    Please see \cref{proof:thm:icl_gd} for a detailed proof.
\end{proof}


As a direct result, the neural networks ${\rm NN}_{\theta}$ constructed earlier is able to approximate the true gradient descent trajectory 
$\{w^l_{\rm GD}\}_{l\geq0}$, defined by $w^0_{\rm GD} = \mathbf{0}$ and 
$w^{l+1}_{\rm GD} = w^l_{\rm GD} - \eta \nabla_w \mathcal{L}_n(w^l_{\rm GD})$ for any 
$l \geq 0$.  
Consequently, \cref{thm:icl_gd} motivates us to investigate the error accumulation under setting 
\begin{align*}
    \bar{w}^{(l)} = 
    {\rm Proj}_{\mathcal{W}} 
    (\bar{w}^{(l-1)} - \eta \nabla \mathcal{L}_n(\bar{w}^{(l-1)}) + \epsilon^{(l-1)}), \quad \bar{w}^{(0)} = \mathbf{0},
\end{align*}
where $\|\epsilon^{(l-1)}\|_2 \leq \eta \epsilon$ represents error terms.
Moreover, \cref{coro:error_ICGD} shows ${\rm NN}_{\theta}$ constructed in \cref{thm:icl_gd} implements $L$ steps ICGD with exponential error accumulation to the true GD paths.

\begin{corollary}[Error for implementing ICGD on $N$-layer neural network]
\label{coro:error_ICGD}
    Fix $L \geq 1$, under the same setting as \cref{thm:icl_gd}, $(2N+4)L$-layer neural networks
    ${\rm NN}_{\theta}$ approximates
    the true gradient descent trajectory 
    $\{w^l_{\rm GD}\}_{l\geq0} \in \R^{D_N}$ with the error accumulation
    $\|\bar{w}^{l}-w^{l}_{\rm GD}\|_2
        \leq L_f^{-1} (1 + n L_f)^l \epsilon$,
    where $L_f = \sup_{w \in \mathcal{W}} \|\nabla^2 \mathcal{L}_N(w)\|_{\rm op}$ denotes the smoothness of $\mathcal{L}_N(w)$ within $\mathcal{W}$.
\end{corollary}
\begin{proof}
    Please see \cref{proof:coro:error_ICGD} for a detailed proof.
\end{proof}



==> 3exp.tex <==




